Performance Guarantee under Longest-Queue-First Schedule in Wireless Networks

Efficient link scheduling in a wireless network is challenging. Typical optimal algorithms require solving an NP-hard sub-problem. To meet the challenge, one stream of research focuses on finding simpler sub-optimal algorithms that have low complexity but high efficiency in practice. In this paper, we study the performance guarantee of one such scheduling algorithm, the Longest-Queue-First (LQF) algorithm. It is known that the LQF algorithm achieves the full capacity region, $\Lambda$, when the interference graph satisfies the so-called local pooling condition. For a general graph $G$, LQF achieves (i.e., stabilizes) a part of the capacity region, $\sigma^*(G) \Lambda$, where $\sigma^*(G)$ is the overall local pooling factor of the interference graph $G$ and $\sigma^*(G) \leq 1$. It has been shown later that LQF achieves a larger rate region, $\Sigma^*(G) \Lambda$, where $\Sigma^ (G)$ is a diagonal matrix. The contribution of this paper is to describe three new achievable rate regions, which are larger than the previously-known regions. In particular, the new regions include all the extreme points of the capacity region and are not convex in general. We also discover a counter-intuitive phenomenon in which increasing the arrival rate may sometime help to stabilize the network. This phenomenon can be well explained using the theory developed in the paper.

==> sections/characterizationofcapacityregion.tex <==
\label{sec:charactercapacityregion}

%The capacity region is a convex polytope in the $|V|$ dimensional
%vector space. Those constraints of the capacity region will
%determine the complexity of the scheduling problem.


%A half-space in the vector space is one of the two parts which are
%separated by a hyperplane. Every half-space can be specified by a
%linear inequality. A convex polytope can be defined as an
%intersection of a set of half-spaces. We call such definition of
%convex polytope half-space representation(H-representation). It has
%been shown that, the minimal H-representation, where the number of
%half-spaces is minimal, is unique. Inequalities that specify all
%those half-spaces in the minimal H-representation defined convex
%polytope.

%The constraints of convex polytope are a set of linear inequalities,
%each of which specifies a half space. The capacity region is
%considered to be the intersection of those half spaces.

%Determining whether an arrival vector is feasible is the same as a
%membership problem of a convex polytope. A feasible problem
%$F(G,\lambda)$ respected to scheduling is defined as follows:
%
%\begin{align}
%F(G, \lambda)=\min \hspace{0.2in} &0\\
% \text {subject to} \hspace{0.2in} &A_G x \leq b \\
%                    &x\ \geq \lambda.
%\end{align}
%Here, $A_G x \leq b$ represents the set of constraints of the
%capacity region. $F(G, \lambda)=0$, when $\lambda$ is in the
%capacity region; $F(G, \lambda)=\infty$, when $\lambda$ is outside
%the capacity region.
The capacity region is a convex polytope in $|V|$ dimensional vector
space. The difficulty of scheduling problem will be affected by the
shape of capacity region. Hence, to study the characterization of
the capacity region is crucial.

\subsection{Extreme Point Perspective}
One way to study convex polytope is to consider all its extreme
points. An extreme point of a convex polytope is a point in the
convex polytope which does not lie in any open line segment joining
two points in the convex polytope. The Krein-Milman theorem
\cite{MKDM40} says that a compact convex polytope is the convex hull
of all its extreme points.

Now, we study the extreme points of the capacity region of graph
$G=(V, E)$. An independent set of a graph $G=(V, E)$ is a subset of
$V$ such that none pair of nodes in the subset are connected with a
link directly. Note that we consider empty set as a trivial
independent set. We find that the set of all extreme points of
capacity region $\Lambda$ has a bijection to the set of all
independent sets of graph $G$.

\begin{lemma} \label{indepextrem}
For an interference graph $G=(V, E)$, the set of all the independent
sets has a bijection to the set of all the extreme points in
$\Lambda$.
\end{lemma}
\begin{proof}
Let $D_E$ be the set of all the independent sets of $G$. Any vector
$\nu \in D_E$ satisfies that $\nu_i=0$ or $\nu_i=1$ for any index
$i$. Since $\nu \in D_E$, there must exist a maximal schedule $\mu$
extended from $\nu$ such that $\nu \leq \mu$ and $\mu \in M_E \in
Co(M_E)$. Hence, $\nu \in \Lambda$ according to the definition.
Suppose $\nu$ is not an extreme point of $\Lambda$, then $\nu=\alpha
\nu^1+ (1-\alpha) \nu^2$ for some $0<\alpha<1$, $\nu^1, \nu^2 \in
\Lambda$ and $\nu^1, \nu^2 \neq \nu$. Since any vector in $M_E$ has
value 0 or 1 in every dimension, $\mu \leq 1$ for every $\mu \in
Co(M_E)$. Thus, $0\leq \nu^1 \leq 1$ and $0\leq \nu^2 \leq 1$. For
any index $i$, if $\nu_i=0$, we must have $\nu^1_i=0$. Otherwise, if
$\nu^1_i>0$, $\nu_i=\alpha \nu^1_i+ (1-\alpha) \nu^2_i \geq \alpha
\nu^1_i
>0$. Symmetrically, $\nu^2_i=0$, if $\nu_i=0$. By similar argument, if
$\nu_i=1$, we derive that $\nu^1_i=\nu^2_i=1$. Since the above holds
for all index $i$, $\nu=\nu^1=\nu^2$, which leads to a
contradiction. Therefore, $\nu$ is an extreme point of $\Lambda$.

Conversely, since $\Lambda$ is a closed region, any extreme point
$\nu$ of $\Lambda$ belongs to $\Lambda$. Then, $\nu \leq \mu$ for
some $\mu \in Co(M_E)$. For an index $i$, if $\nu_i
>0$, then $\nu_i = \mu_i$. Otherwise, we let $t=\mu_i-\nu_i>0$.
Then, we can create $\bar{\nu}$ and $\tilde{\nu}$ such that
$\bar{\nu}_j=\tilde{\nu}_j=\nu_j$ for $j \neq i$. And we can find an
$\epsilon>0$ letting $\bar{\nu}_i=\nu_i-\epsilon t \geq 0$,
$\tilde{\nu}_i=\mu_i \geq 0$. Since $0 \leq \bar{\nu} \leq
\tilde{\nu} \leq \mu$, $\bar{\nu}, \tilde{\nu} \in \Lambda$. We find
that $\nu=\frac {1} {1+\epsilon} \bar{\nu}+ \frac{\epsilon}
{1+\epsilon} \tilde{\nu}$, which implies $\nu$ is not an extreme
point.  Hence, $\nu_i=0$ or $\nu_i=\mu_i$, for all index $i$. We now
show that $\nu_i=0$ or $\nu_i=1$, for all index $i$. Suppose not, we
have $\mu=a_1\mu^1+a_2\mu^2+...+a_k \mu^k$ and $\mu^1, \mu^2,...
\mu^k \in M_E$, $a_1, a_2,..., a_k>0$, $a_1+a_2+...+a_k=1$. Let
$\nu^j_i=0$ if $\nu_i=0$; $\nu^j_i=\mu^j_i$ otherwise, for all $0
\leq j \leq k$. Because $\mu^j \in M_E$, we have $\nu^j_i=0$ or
$\nu^j_i=1$. It is easy to check that $\nu=a_1 \nu^1+a_2 \nu^2+...
+a_k \nu^k$. Since $\nu$ is an extreme point of $\Lambda$,
$\nu^1=\nu^2=... =\nu^k$. Thus, $\nu_i=1$ or $\nu_i=0$, for all
index $i$. Therefore, every extreme point can be mapped to an
independent set.
\end{proof}

We take graph of triangle as an example to illustrate the
relationship between independent sets of a graph and extreme points
of capacity region. The graph is showed in the left part of figure
\ref{fig:extrindep}. Since the three nodes in the graph interfere
with each other, there are at most one node been selected in every
independent set. There are four independent sets in this graph: $(1,
0, 0), (0, 1, 0), (0, 0, 1), (0, 0, 0)$. Correspondingly, we can see
in the right part of figure \ref{fig:extrindep}: the four vectors
are exactly those extreme points of the capacity region in 3
dimensional space.

\begin{figure}[htbp]
  \begin{center}
    \includegraphics[width=3.2in]{fig/extremindep.eps}
  \end{center}
  \caption{Relationship between graph independent set and extreme point of capacity region. Left:
  the triangle graph; Right: the capacity region.}
  \label{fig:extrindep}
\end{figure}

Of cause, we can obtain the capacity region of graph $G$ by
calculating the convex hull of all the extreme points. Those extreme
points are the vectors representing independent sets of the graph
$G$. When the number of independent sets of graph is small, this
algorithm can be efficient. For example, if $G=(V, E)$ is a clique,
there are only $|V|+1$ independent sets. In such a case, the
capacity region is easy to calculate.

Unfortunately, the number of independent sets in a graph is
generally as large as exponential respected to the number of nodes
in the graph. Hence, in general, the number of extreme points is
exponential respected to the number of nodes in the graph. In
general graph, even obtaining those extreme points is too
complicated.

Note that, the exponential number of independent sets does not
require the graph to be very complicated. Consider a graph composed
by a line of $n$ nodes. In any maximal independent set, there are at
least $\lfloor\frac{n-1}{3}\rfloor+1$ number of nodes. Between two
consecutive nodes in maximal independent set, there can be either
one node or two nodes. Hence, the number of maximal independent sets
is exponential respected to the number of nodes in this graph. Thus,
the number of independent sets of this graph is exponential.

%$\noindent {\bf Fact \; :}$ Consider a graph composed by a line of
%$n$ nodes. When $n$ is large, there are exponential number of
%maximal independent sets. In any maximal independent set, there are
%at least $\lfloor\frac{n-2}{3}\rfloor+1$ number of nodes. Between
%two consecutive nodes in maximal independent set, there can be
%either one node or two nodes. Hence, the number of maximal
%independent sets is exponential respected to the number of nodes in
%this graph.
\subsection{Constraints Perspective}
Besides extreme points representation, convex polytope can also be
considered as the intersection of half spaces. Those half spaces are
one side of a hyperplane in vector spaces. Each of those hyperplane
corresponds to a facet of the convex polytope. Half spaces can also
be written as linear constraints mathematically. Since the convex
polytope is the intersection of half spaces, one point is in the
convex polytope if and only if it satisfies all those linear
constraints corresponding to those half spaces.

The number of constraints of a convex polytope is smaller than the
number of extreme points of it. One linear optimization problem may
have exponential number of extreme points respected to the number of
constraints. Simplex method is not polynomial respected to the size
of the problem, because it may enumerate all the extreme points of
the convex polytope. However, it is well known that ellipsoid
algorithm can solve the problem polynomially respected to the number
of constraints. This phenomenon suggests us to consider the
constraints instead of extreme points of capacity region.

Suppose we formulate the capacity region as a feasibility problem
with those linear constraints corresponding to those half spaces
that determine the capacity region. If the number of those
constraints is polynomial respected to the number of nodes in the
graph, the capacity region can be obtained polynomially respected to
the number of nodes in the graph as well by applying ellipsoid
algorithm.

Given $x$ is an arrival vector in the capacity region, there are two
classes of constraints that are necessary. One is called clique
constraints which force the summation of arrival for any clique less
than or equal to one. Since every time instance at most one node in
a clique can be served, those constraints are necessary.
\begin{align*}
\sum_{i \in Q} x_i \leq 1, \hspace{0.1in} \text{for all clique}
\hspace{0.1in} Q \hspace{0.1in} \text{in} \hspace{0.1in}G.
\end{align*}
Another class of necessary constraints for the arrival is
nonnegativity constraints, which force the arrival rate for any node
to be nonnegative.
\begin{align*}
x_i \geq 0, \hspace{0.2in} \forall i.
\end{align*}

Article \cite{VC75} shows that, for perfect graph, clique
constraints and nonnegative constraints are sufficient to determine
the capacity region.


\begin{theorem} \cite{VC75} \label{thm:capacityperfect}
When graph $G$ is perfect, the nonnegativity constraints and the
clique constraints are sufficient to determine the capacity region
$\Lambda$.
\end{theorem}

\begin{corollary}
When graph $G=(V, E)$ is a tree, $x_i+x_j\leq 1$ for all $(i,j) \in
E$ and the nonnegative constraints $x_i \geq 0$ for all $i \in V$
determine the capacity region $\Lambda$.
\end{corollary}

This corollary is true simply because the set of cliques in a tree
equals the set of pairs of neighbors. Since there are only $|V|-1$
links in a tree, the number of clique constraints is $|V|-1$ which
is polynomial. The number of those nonnegative constraints is $|V|$.
So, the number of constraints of capacity region for a tree is
polynomial.

\begin{figure}[htbp]
  \begin{center}
    \includegraphics[width=2.6in]{fig/perfect.eps}
  \end{center}
  \caption{Constrains for capacity of graphs. Left:
  the graph of a Line; Right: the graph of Pentagon.}
  \label{fig:perfect}
\end{figure}

The left side of figure \ref{fig:perfect} is a line which is
perfect. The clique constraints as $x_i+x_j \leq 1$ and nonnegative
constraints $x_i \geq 0$ determine the capacity region. In the
previous section, we have shown the number of extreme points of the
capacity region of this graph is exponential respected to the number
of nodes. Here, we justify that the number of constraints of the
capacity region of this graph is polynomial respected to the number
of nodes.

However, the number of constraints of capacity region is not always
polynomial. For example, let graph $G$ be the complement graph of a
line $\bar{G}$. Every maximal clique in $G$ corresponds to a maximal
independent set in $\bar{G}$. Hence, the number of maximal cliques
in $G$ is exponential which makes the number of clique constraints
exponential as well. Though theorem 9.4.3 in \cite{MLA85} indicates
that the capacity region of perfect graph can be calculated in
polynomial time, the algorithm is not easy to apply in the wireless
networks scheduling problem.

Another problem is that clique constraints and nonnegative
constraints are not sufficient when the graph is not perfect. The
right side of figure \ref{fig:perfect} is a pentagon which is not
perfect. We can check that vector $(1/2, 1/2, 1/2, 1/2, 1/2)$
satisfies the clique constraints and nonnegative constraints. But,
this vector is outside the capacity region.

\subsection{Reduced Dimensional Subspace Perspective}
For graph $G=(V, E)$, the capacity region $\Lambda$ is a convex
polytope in $|V|$ dimensional vector space. The complexity of
calculating $\Lambda$ may grow very fast with the increasing of
$|V|$. Projecting the arrival rate in some reduced dimensional
subspaces may provide an easier way to study the capacity region.

Roughly speaking, a network is stable if and only if every subset of
the network is stable. In most cases, the work loads for different
links of the whole network vary a lot. Some set of nodes may have
very light traffic which will not create instability problem. In
such case, to study the network excluding those nodes with light
traffic is enough.

\begin{theorem} \label{thm:subsetcapacity}
Given a interference graph $G = (V, E)$, the arrival rate vector
$\lambda \in \Lambda$ if and only if for all $S \subseteq V$,
$[\lambda]_S \in \Lambda_S$. Likewise, $\lambda \in \Lambda^o$ if
and only if for all $S \subseteq V$, $[\lambda]_S \in \Lambda^o_S$.
\end{theorem}

\begin{proof}
Suppose $\lambda \in \Lambda$, then $\lambda \leq \mu$ for some $\mu
\in Co(M_V)$. For any subset $S \subseteq V$, there must exist a
vector $\nu \in Co(M_S)$ such that $[\mu]_S \leq \nu$. Then,
$[\lambda]_S \leq \nu$. Hence, $[\lambda]_S \in \Lambda_S$. The
other direction is true by taking $S=V$. The interior point
statement can be proved similarly.
\end{proof}



%Set $\sigma$ local pooling is studied in \cite{BCY09}. We
%
%\begin{definition}
%Given a non-empty set $L \subseteq E$, we say $L$ has a \em{set
%$\sigma$-local pooling} factor $\sigma_L^*$ if the following holds.
%\begin{align}
%\sigma_L^* := & \sup \{\sigma \ | \ \sigma \in \Theta_L \}
%\label{eq:setsigsup}\\
%:= & \inf \{\sigma \ | \ \sigma \in \Theta_L^c\}.
%\label{eq:setsiginf}
%\end{align}
%\end{definition}
%
%The optimal solution of the following problem has been showed to be
%the set $\sigma$ local pooling factor:
%
%\begin{align*}
%\min_{\sigma, \mu_L, \nu_L} & \ \sigma \\
%\text{subject to } & \ \sigma \mu_L \geq \nu_L \\
%& \mu_L, \nu_L \in Co(M_L).
%\end{align*}
%
% Consider the dual problem for
%computing the set $\sigma$-local pooling factor:
%\begin{align*}
%\textbf{(Dual)} \hspace{0.2in} \max_{x \geq 0, w} & \ w \\
%\text{subject to } & \ x' M_L \leq e_{c(L)}' \\
%& \ x' M_L \geq w e_{c(L)}'.
%\end{align*}
%The weight assignment $x_L^*$ is optimal when $w$ is maximized.
%
%Consider an arrival vector $\lambda$ for the network. The membership
%problem is to determine whether $\lambda$ is in the capacity region.
%
%\begin{lemma}
%Arrival vector $\lambda$ is strictly inside the capacity region if
%and only if $(x_L^*)' [\lambda]_L < 1$ for all subset $L$.
%\end{lemma}
%\begin{proof}
%Since $\lambda$ is inside the capacity region, $\lambda < \mu$ for
%some $\mu \in Co(M_E)$. For each subset $L \in E$, there must exist
%a $\nu \in Co(M_L)$ such that $[\mu]_L \leq \nu$. Then, we have
%$[\lambda]_L < \nu$, which implies that $(x_L^*)' [\lambda]_L <
%(x_L^*)' \nu \leq 1$.
%
%Now, suppose $\lambda$ is outside the capacity region.
%\end{proof}

